Infighting in the Dark: Multi-Label Backdoor Attack in Federated Learning

Federated Learning (FL), a privacy-preserving decentralized machine learning framework, has been shown to be vulnerable to backdoor attacks. Current research primarily focuses on the Single-Label Backdoor Attack (SBA), wherein adversaries share a consistent target. However, a critical fact is overlooked: adversaries may be non-cooperative, have distinct targets, and operate independently, which exhibits a more practical scenario called Multi-Label Backdoor Attack (MBA). Unfortunately, prior works are ineffective in the MBA scenario since non-cooperative attackers exclude each other. In this work, we conduct an in-depth investigation to uncover the inherent constraints of the exclusion: similar backdoor mappings are constructed for different targets, resulting in conflicts among backdoor functions. To address this limitation, we propose Mirage, the first non-cooperative MBA strategy in FL that allows attackers to inject effective and persistent backdoors into the global model without collusion by constructing in-distribution (ID) backdoor mapping. Specifically, we introduce an adversarial adaptation method to bridge the backdoor features and the target distribution in an ID manner. Additionally, we further leverage a constrained optimization method to ensure the ID mapping survives in the global training dynamics. Extensive evaluations demonstrate that Mirage outperforms various state-of-the-art attacks and bypasses existing defenses, achieving an average ASR greater than 97\% and maintaining over 90\% after 900 rounds. This work aims to alert researchers to this potential threat and inspire the design of effective defense mechanisms. Code has been made open-source.

==> sec_cr/4_methodology_before.tex <==
\section{Methodology}
\label{Sec: Methodology}
To formulate the attack scenario, we first introduce the threat model. Driven attack intuitions, we propose two methods that enable attackers to construct an efficient and persistent ID mapping without cooperation.
\subsection{Threat model} 
\noindent\textbf{Adversaries’ Capabilities and knowledge}. We consider a FL system running image classification tasks and assume that adversaries are FL participants, which enables attackers to control their own local datasets and training processes. Note that adversaries do not have access to any information regarding benign clients or other adversaries, including but not limited to datasets, models, target classes.
% , which means they have the full control over the training process and have the access to its local datasets. Besides, attackers also have the access to the global model if they are selected to the have full access to their local datasets and training processes. The adversaries also have access to the global model weights and predictions. However, adversaries do not have access to any information of benign clients or other adversaries, including their datasets, models, target classes and others.
% the dataset and models of other clients or adversaries. Different from previous work, in which multiple attacker target labels are consistent, we define that the attacker has no information about the other attackers.

\noindent\textbf{Adversaries' goal.} Adversaries aim to plant a backdoor into the global model that makes it misclassify backdoor data to a specific class while leaving other tasks unaffected.

\begin{figure*}
    \centering
    \setlength{\abovecaptionskip}{2 mm}    \includegraphics[width=1\linewidth]{Figs/framework_v4.0.pdf}
    \caption{The workflow of Mirage. \textbf{Step 1}: Train an OOD sample detector $\theta_{Detector}$. \textbf{Step 2}: Construct ID mapping by maximizing misclassification probabilities of backdoor samples on the detector. \textbf{Step 3}: Tighten backdoor distribution by minimizing the feature similarities between backdoor samples and benign samples. \textbf{Step 4}: Optimize the trigger by minimizing $L_{Enhance}$ and $L_{detector}$. }
    \label{Fig: workflow}
    \vspace{-4 mm} 
\end{figure*}
% 本章中，我们详细描述我们所提出的框架，其通过建立后门特征到干净分布之间的干净映射来完成无串通情况下的MBA.
%在本章节，我们展示了所提出框架的细节，其允许攻击者构建从后门特征到目标类别分布的分布内映射，以此使得攻击者可以无惧其他攻击者的潜在抵消
\subsection{Overview of Mirage}
Following the attack intuition, our objective is to construct an ID mapping to bridge the backdoor features and distribution of target class, thereby freeing attackers from the exclusion of using similar backdoor activation paths. This presents two significant challenges: how to construct a qualified ID mapping and how to maintain it. To address these challenges, we propose Mirage, the first multi-label backdoor attack in FL, which enables attackers to non-cooperatively compromise the global model by constructing an ID mapping between the backdoor features and target distributions. As illustrated in Fig.~\ref{Fig: workflow}, Mirage introduces two components to construct an effective and persistent ID backdoor mapping. On one hand, we propose a backdoor optimization method based on adversarial adaptation, which constructs the ID mapping by maximizing the misclassification probability of a well-designed backdoor sample detector. On the other hand, we deploy a constrained optimization strategy to tighten the backdoor distribution, ensuring its survival in the global training dynamics. Next, we provide details of each component.
% which introduces two carefully designed adaption goals to adversarially optimize the backdoor trigger for attackers, thus building the bridge between backdoor features and the target class's features. The workflow of Mirage is illustrated in Fig~\ref{Fig: workflow}. Specifically, we first introduce an adversarial loss, which optimize the backdoor pattern by maximizing the misclassification probability of a well-trained OOD-backdoor detector to address the former challenge. In order to further enhance the backdoor mapping, we deploy a constrained optimization strategy together with the adversarial loss. 


% In this section, we present the details of our proposed framework, which allows an attacker to construct an ID mapping from backdoor features to the target class distribution, thereby allowing the attacker no fear for the potential mitigation of other attackers. To achieve this objective, two challenges remain to be addressed: how to construct the qualified ID mapping and how to maintaining the ID mapping.


% In this section, we present the details of our proposed framework, which backdoor the FL model by mapping the backdoor feature to the 
% which aims to allowing the adversaries to successfully launch multi-label backdoor attacks in FL without collusion. Following the attack intuition, our goal is to avoid the conflict of backdoor activation paths of non-collusion attackers by constructing ID mappings towards trigger patterns and the targeted clean distributions. This poses two significant challenges for building qualified ID mappings. On the one hand, backdoored samples should reveal the ID characteristics of the target class. On the other hand, the ID mapping effectiveness should be maintained over time. 

% To address these challenges, a novel framework is proposed, which adversarially optimizing the trigger pattern so that the backdoored sample can activate the clean activation path of the target class. 

% Our primary objective is to optimize the backdoor trigger in a way that allows trigger pattern to present the key feature of the target class. Thus, the backdoor samples can be mistakenly identified by the model as clean class samples with noise, activating the clean paths of the target class.





% 我们用后门特征构成目标类的关键特征，然后原始样本的特征相当于噪声样本，我们本地训练的时候相当于利用干净样本加噪声。这样的话，解决挑战1就是利用detector来对抗生成目标类的关键特征，然后挑战2就是端到端增强，相当于加了干净特征加了噪声后，使模型对目标类进行鲁棒训练
\subsection{Effective ID Mapping Construction}
\label{Subsec: ID mapping construction}
% 如何解决挑战1：构建ID mapping
To address the first challenge, we aim to adversarially optimize the trigger pattern to make it has the ability of constructing the ID mapping. In order to optimize the trigger, we employ an OOD sample detector to determine whether a backdoored sample is an OOD sample and further optimize the trigger pattern to fool the detector. This introduces another problem: how can an attacker obtain an accurate detector? Previous research suggests training a new model as the detector \cite{Advdoor_zhang_2021}. However, retraining the detector with each update of the trigger incurs significant computational overhead, and its effectiveness is limited by the local samples. These shortcomings prompt us to seek another solution to obtain an detector that is both effective and lightweight for updates. Recall that the FL training process allows clients to obtain the latest global model, which contains a well-trained feature extractor. Consequently, we consider leveraging the feature extractor of the global model as the primary component and training a binary classifier to distinguish the OOD samples. Such an approach is a common practice in transfer learning, consume only a few computing resources, and require little data.

% Recall the tradition backdoor attacks again, they focus on building a shortcuts path towards the target class, produces an OOD mapping to the clean samples, which means that the global model,especially the feature extractor, process the clean sample and backdoored sample in different way. Thus, a directly solution for detector is that we can leverage the feature extractor of global model as the major component of detector and train a binary-classifier to discriminate the clean samples.
In order to obtain an accurate detector, we first prepare the dataset for training. The local dataset for each attacker can be divided into $D_{cln}=\{(x,y)\in D_{att})|+\}$ and $D_{bd} = \{(x\oplus\delta,y)\in D_{att})|-\}$, where $+$ indicates the ground truth label of a sample is $c$, and $-$ is the opposite and $\delta$ represents the trigger pattern. Then, the detector dataset $D_{detector}$ ($D_{d}$ for short) is composed as follows:
\begin{equation}
\begin{array}{rr}
   D_{d} = \{(x,-) \mid x \in D_{bd}\} \cup \{(x,+ ) \mid x \in D_{cln}\},
\end{array}
\label{Equ: detector dataset construct}
\end{equation}

% In order to obtain an accurate detector, the dataset is also a necessary precondition. We directly divide the local dataset of an attacker to $D_{clean}=\{(x,y)\in D_{attacker})|y=c\}$, where $c$ is the target class for the attacker. The left samples are making up to $D_{backdoor} = \{(x\oplus\delta,y)\in D_{attacker})|y\neq c\}$ where $\delta$ represent the trigger pattern. Further, the detector dataset $D_{detector}$ is composed as follows:
% \begin{equation}
% \begin{array}{ll}
%    D_{detector} =  \\
%         \{(x,false) \mid x \in D_{backdoor}\} \cup \{(x,true) \mid x \in D_{clean}\}.
% \end{array}
% \label{Equ: detector dataset construct}
%  % \{(x,false) \mid x \in D_{backdoor}\} \cup \{(x,true) \mid x \in D_{clean}\}.
% \end{equation}


To make the ID mapping construction more effective and flexible, we adopt an adversarial training-like method to optimize the trigger pattern. Specifically, $\theta_{detector}$ is trained on the $D_{detector}$ to differentiate between clean and backdoored samples by minimizing the binary cross-entropy (BCE) loss. 

Concurrently, the trigger is optimized to fool the detector by maximizing the binary classification loss. Such a min-max game equips the trigger with the ability to activate the clean activation path of the target class in the global model, naturally avoiding conflicts with other attackers. The min-max process is mathematically described as:
\begin{equation}
\begin{array}{c}
\delta=\underset{\delta}{\ \operatorname*{argmin}} \ \mathbb{E}_{(x,y)\sim D_{detector}}[\mathcal{L}(x,+,\theta)|y=-]
\\
    s.t.\ \theta = \ \underset{\theta}{\operatorname*{argmin}}\  \mathbb{E}_{(x,y)\sim D_{detector}}[\mathcal{L}(x,y,\theta)]
\end{array}
\end{equation}
where $\theta$ is the parameters of the detector, with its feature extractor frozen and parameterized by the weights of the global model, $\mathcal{L}$ is the BCE loss. To better implementation, we replace the maximization problem with minimizing the BCE loss of misclassification for the backdoored samples.

% Specifically, we aim to train a OOD detector $\theta_{detector}$ to discriminate whether a sample is backdoored, and further adversarial optimize the trigger to fool the detector. Previous research proposed to train an MLP as the discriminator, which is not appropriate here, since iterative optimize the trigger pattern request the detector have sufficient data samples which is not realistic in FL. 


% we adopt an adversarial training-like method to optimize the trigger pattern to build the bridge between the backdoored feature and target clean distribution.
% % 利用对抗训练的思想，优化trigger，具体是构建一个OOD探测器，通过不断对trigger优化，来使得trigger可以表现出目标类的干净特征
% Specifically, we aim to train an OOD detector $\theta_{detector}$ to discriminate whether a sample is backdoored, and further adversarial optimize the trigger pattern to fool the detector. To achieve this, a binary detector should be trained and updated with trigger.

% % 如何构建detector - 数据集构建



% After that, we 
% % 如何构建训练集
% % 对抗优化的目标
% In this subsection, we detail the design of the OOD detector $\theta_{detector}$ and how can we optimize the trigger pattern to ensure the backdoored sample that are in-distribution.


\subsection{Persistent ID Mapping Enhancement}
\label{Subsec: ID mapping enhancement}
% 为什么要做增强： 因为目前的受限于攻击者本地的数据，训练出的detector会有欠缺，也就是不能表现出较强的后门特征

% 这是因为detector受限于本地样本不足以及目标类样本的表征之间存在一定差异，导致先前生成的trigger无法使所有被后门的样本处于分部内，由于我们采用激活干净神经通路的方式植入后门，这些样本无法有效的激活目标通路，造成了攻击的成功率不及预期。在以往的工作中同样存在这样的情况，一些工作提出利用GAN或者生成模型来丰富本地数据，或者使用KDE方法估计目标分布，然后通过数据增强来增加本地样本，但是这种方式极大的增加了计算开销。
Although using an OOD detector and an adversarial strategy restricts the trigger pattern $\delta$ to reveal the ID feature, our empirical results indicate that the backdoored samples still do not meet our expectations. This is because the adversarial strategy does not constrain the tightness of backdoor mapping, which causes the margin-distributed backdoored samples not in-distribution anymore with the dynamic changes of training and failing to activate the target activation path. One promising solution is to leverage distribution estimation methods, like KDE \cite{KDE_sheather_1991}, to obtain the actual distribution of the target class and use data augmentation to generate samples to improve the effectiveness of the detector. Although it has been proven effective, it requires countless computing resources. Therefore, we introduce a constrained optimization method to enhance the ID mapping by tightening the distribution of backdoored samples. Since the adversarial strategy successfully constructs the ID mapping, we aim to “push” the backdoor distribution to make it tighter. Specifically, we minimize the similarities between clean samples $x$ and their corresponding backdoored samples $x \oplus \delta$, allowing the backdoored sample to deviate as much as possible from the original distribution. Additionally, we establish the direction by minimizing the loss of the backdoor samples on the global model. Formally, it can be formulated as the following optimization problem:
\begin{equation}
\begin{array}{r}
 \delta = \operatorname{argmin}\ \operatorname{CS}[(\theta_{f}(x),\theta_{f}(\hat{x})]  +  \operatorname{CE}(\hat{x},\hat{y}, \theta)
\end{array}
\end{equation}
where $\theta_{f}$ represents the feature extractor of the global model $\theta$. $\hat{x} = x \oplus \delta, x\in D_{att}$, $\oplus$ is the backdoored operator. $\operatorname{CS(\cdot)}$ and $\operatorname{CE(\cdot)}$ represent the Cosine-similarity and the Cross-entropy loss, separately. Therefore, the backdoor distribution can be tightened into the target distribution and live within the global training dynamics.


% Specifically, we aim to maximize the difference between the clean sample $x$ and its corresponding backdoored sample $x \oplus \delta$, allowing the backdoored sample to deviate as much as possible from the original distribution. Additionally, we maintain the tightness of the backdoor mapping in the target distribution by minimizing the loss of the backdoor samples on the global model, i.e., enhancing their ID mapping in the target distribution. Formally, the ID mapping enhancement can be formulated as the following optimization problem:


We summarized Mirage in Algorithm~\ref{Algo: Mirage}, and the detailed description is provided in Appendix ~\ref{Appendix: Algorithm Outline}.

\begin{algorithm}[h]

\caption{Mirage at $i$-th attacker.}

\label{Algo: Mirage}
\KwData{$\theta_t,\theta_{detector},\theta_{fe},\mathcal{D}_i,\delta,\eta, c, E$.}

$\theta_t^{i} = \theta_t $\;
\textit{/* Trigger adversarial adaption*/}

\For{epoch $e=1$, \dots, $E$}{
    Generate $D_{detector}$ by Eq~\ref{Equ: detector dataset construct}\;
    $\theta_{detector}= \underset{\theta}{\operatorname*{argmin}}\  \mathbb{E}_{(x,y)\sim D_{detector}}[\mathcal{L}(x,y,\theta_{detector})]$\;

    \For{batch $\mathcal{B} \in D_i$}{
    $\mathcal{L}_{detector} = \frac{1}{|\mathcal{B}|}\sum_{(x,y)\in\mathcal{B}}\mathcal{L}_{BCE}(x\oplus\delta, + ,\theta_{detector})$\;

    $\mathcal{L}_{Enhance} = \frac{1}{|\mathcal{B}|}\sum_{(x,y)\in\mathcal{B}}\mathcal{L}_{CE}(x\oplus\delta, \hat{y},\theta_t^{i})\hfill$ \\ 
    $ \hfill+  \mathcal{L}_{CS}((\theta_{fe}(x),\theta_{fe}(x \oplus \delta));$
    
    $\delta\leftarrow \delta - \eta \cdot \nabla_{\delta}(\mathcal{L}_{detector} + \mathcal{L}_{Enhance});$
    }
}
\textit{/* Local training*/}

Get the poisoned local dataset $\mathcal{D}_i^{poison}$ with $\delta$\;

Local optimize $\theta_t^{\prime}$ on $\mathcal{D}_i^{poison}$\;

$\boldsymbol{\Delta}_i^{t+1}=\theta_t-\theta_t^\prime$\;

Upload $\boldsymbol{\Delta}_i^{t+1}$ to the server\;

\end{algorithm}
% \begin{algorithm}[H]
% \caption{Mirage at $i$-th attacker.}
% \label{Alg: Mirage}
% \begin{algorithmic}
% \STATE \textbf{Input:} $\theta_t,\theta_{detector},\theta_{fe},\mathcal{D}_i,\eta_{trigger},\delta,\eta,\lambda_1,\lambda_2, c, E.$
% \STATE$\theta_t^{i} = \theta_t $
% \STATE \textit{/* Trigger adversarial adaption*/}
% \FOR{round $k=1$, \dots, $K$} % 本地trigger search time
%    \STATE   Generate $D_{detector}$ by Eq~\ref{Equ: detector dataset construct}.
%    \STATE   $\theta_{detector}= \underset{\theta}{\operatorname*{argmin}}\  \mathbb{E}_{(x,y)\sim D_{detector}}[\mathcal{L}(x,y,\theta_{detector})]$
%    \FOR{batch $\mathcal{B} \in D_i$}
%    \STATE $\mathcal{L}_{detector} = \frac{1}{|\mathcal{B}|}\sum_{(x,y)\in\mathcal{B}}\mathcal{L}_{BCE}(x\oplus\delta, true,\theta_{detector})$
   
%    \STATE $\mathcal{L}_{Enhance} = \frac{1}{|\mathcal{B}|}\sum_{(x,y)\in\mathcal{B}}\mathcal{L}_{CE}(x\oplus\delta, \hat{y},\theta_t^{i})\hfill$ \\ 
%     $ \hfill+  \mathcal{L}_{CS}((\theta_{fe}(x),\theta_{fe}(x \oplus \delta))$
%     $\delta\leftarrow \delta - \eta_{trigger}\nabla_{\delta}(\lambda_1\mathcal{L}_{detector} + \lambda_2\mathcal{L}_{Enhance})$
    
%    \ENDFOR
% \ENDFOR
% \STATE \textit{/* Local training*/}
% % poison local dataset
% \STATE Get the poisoned local dataset $\mathcal{D}_i^{poison}$ with $\delta$.
% \STATE Local optimize $\theta_t^{\prime}$ on $\mathcal{D}_i^{poison}$.
% % \FOR{epoch $e=1$, \dots, $E$}
% % \FOR{batch $\mathcal{B} \in \mathcal{D}_i^{poison}$}
% % \STATE  $\theta_t^{\prime}\leftarrow\theta_t^{\prime}-\eta \nabla_{\theta}\frac{1}{|\mathcal{B}|}$
% % \ENDFOR
% % \ENDFOR
% \STATE $\boldsymbol{\Delta}_i^{t+1}=\theta_t-\theta_t^\prime$
% \STATE Upload $\boldsymbol{\Delta}_i^{t+1}$ to the server.
% \end{algorithmic}
% \label{Algo: Mirage}
% \end{algorithm}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Detail workflow.pdf}
%     \caption{The detail workflow for attacker.}
%     \label{Fig: detail workflow on attacker }
%     \vspace{-5mm}
% \end{figure}
